Fast algorithms for Jacobi expansions via nonoscillatory phase functions

We describe a suite of fast algorithms for evaluating Jacobi polynomials, applying the corresponding discrete Sturm-Liouville eigentransforms and calculating Gauss-Jacobi quadrature rules. Our approach is based on the well-known fact that Jacobi's differential equation admits a nonoscillatory phase function which can be loosely approximated via an affine function over much of its domain. Our algorithms perform better than currently available methods in most respects. We illustrate this with several numerical experiments, the source code for which is publicly available.

==> acknowledgments.tex <==
\begin{section}{Acknowledgments}
JB was supported in part by a UC Davis Chancellor's Fellowship.
%% The author is grateful to Zydrunas Gimbutas of NIST Boulder
%% for providing his arbitrary precision arithmetic codes
%% for evaluating the associated Legendre functions
%% of large integer degrees and orders via the three-term recurrence relations
%% they satisfy.
%% This work was supported in part by a UC Davis Chancellor's Fellowship.
\end{section}


==> junk <==

%% we use the Fast Fourier transform and this  choice of 
%% approximation is more conducive to the use of the 

%% because we the matrix whose $(j,k)$ entry is 
%% %
%% \begin{equation}
%% \exp\left(i t_j (k-1)\right)
%% \end{equation}
%% %
%% can be applied rapidly with a nonuniform fast Fourier tranfsorm



%% makes use of the Fast Fourier transform and this choice
%% of approximation of 
%% We do not prove a rigorous bound on $r$ here, nor on the rank
%% of (\ref{introduction:matrix})
%% (see, though, Figure~\ref{figure:transform2} in Section~\ref{section:experiments:transform}).
%% Moreover, as far as we the authors are aware, no such bound is known.
%% This is not on account of lack of interest in the subject, however.  Bounds of this
%% sort would be useful in establishing the asymptotic complexity
%% of certain widely used  numerical methods based on butterfly algorithms
%% (such as the scheme of  \cite{tygertIII} for the rapid application of the spherical
%% harmonic transform).

%
%

%
and $\otimes$ denotes the Hadamard product.  The Hadamard product
of two matrices is the matrix obtained through entrywise multiplication.
%% then obviously
%% %
%% \begin{equation}
%% \mathcal{J}_n = 
%% F \otimes  \left(D \cdot R\right),
%% \end{equation}
%% %
%% where

%
%
$D$ is an $n \times r$ matrix and $R$ is an $r \times k$ matrix.
{\bf need to interpolate $R$}
and $A \otimes B$ denotes the Hadamard product of the mari
(that is, entrywise multiplication).  The matrix
$F$ is 

Since $M_\nu$ and $M_t$ are on the order
of $\log\left(N_{\mbox{\tiny max}}\right)$,
the cost of  constructing the interpolative decompositin of 
the matrix (\ref{precomp:matrix})  via the procedure of
\cite{Cheng-Gimbutas-Martinsson-Rokhlin} is
$\mathcal{O}\left(\log^3\left(N_{\mbox{\tiny max}}\right)\right)$.
We note, though, that in all of the numerical experiments of this paper,
the cost of computing the representations of $\psi^{(a,b)}$
and $M^{(a,b})$ dominated the running time of the precomputation
procedure described in this section.

THe procedure just described is inspired by the approach 
of \cite{} for the application of the nonuniform FFT.



%% This is done in two steps.  First, for each $k=1,\ldots,r$,
%% we use Chebysev interpolation  to evaluate 
%% the function
%% %
%% \begin{equation}
%% M^{(a,b)}(x,\gamma_{s_k})
%% \exp\left(
%% i \left(
%% \psi\left(x,\gamma_{s_k}\right) - x \gamma_{s_r}
%% \right)
%% \right),
%% \end{equation}
%% %
%% for $x=t_1,\ldots,t_n$ given its values at the nodes $x=\tau_{1},\ldots,\tau_{M_t}$.
%% The latter collection of values comprise one of the columns of the matrix $B^{(1)}$.
%% We scale each of the former by
%% %
%% \begin{equation}
%% \exp\left(
%% i 
%% (x_j-t_j) \gamma_{s_k}
%% \right).
%% \end{equation}
%% %
%% in order to calculate the $(j,k)$ entry of  $D$.  



We note have that
%
\begin{equation}
,
\end{equation}
%
where  

%% %
%% \begin{equation}
%% M^{(a,b)}(t,\gamma_{s_k})
%% \exp\left(
%% i \left(
%% \psi\left(t,\gamma_{s_k}\right) - t \gamma_{s_k}
%% \right)
%% \right),
%% \ \ \ t = \tau_1,\ldots,\tau_{M_t},
%% \end{equation}
%
 constitute the entries  of the $k^{th}$ column
of the matrix 
from $t = \tau_1,\ldots,\tau_{M_t}$ to the values of this function
%
\begin{equation}
\exp\left(
i \left(
\psi\left(t_j,\gamma_{s_k}\right) - t_j \gamma_{s_k}
\right)
\right)
\end{equation}
%
%
Each column of the matrix  $A^{(1)}$

%% If the user desires to evaluate $\tilde{P}_n^{(a,b)}$ at points
%% closer to $0$ and $\pi$, then
%%  the asymptotic expansion 
%% %% (\ref{asym:p}) and the connection formula
%% %% %
%% %% \begin{equation}
%% %% \tilde{P}_n^{(a,b)}(\pi -t) = (-1)^n \tilde{P}_n^{(b,a)}(t)
%% %% \end{equation}
%% %
%% can be used to do so.  The principal difficulty with using this expansion --- that
%% its higher order coefficients are not known explicitly --- is easy to overcome in this
%% regime since the Taylor series of its coefficients around $0$ can be calculated
%% with relative ease.  


%% and, by a slight abuse of terminology, we will refer to it 
%%  as the nonoscillatory phase function for Jacobi's differential
%% equation (recall that the phase function is only determined up to an integer
%% multiple of $2\pi$).

%% It is well-known that 
%% %
%% \begin{equation}
%% \left(J_a(t)\right)^2
%% +
%% \left(Y_a(t)\right)^2
%% \sim
%% \frac{2}{\pi}
%% \left(
%% \frac{1}{t }+ 
%% \frac{4a^2-1}{8t^2} + \frac{3(9-40a^2+16a^4)}{128t^5} + \cdots \right)
%% %% \frac{5\left(64a^6-560a^4+1036a^2-225\right)}{1024t^7}+ 
%% %% \frac{35\left(256 a^8-5376 a^6+31584 a^4-51664 a^2+11025\right) }{32768t^9}+\cdots\right)
%% \ \ \mbox{as} \ \ t \to \infty
%% \end{equation}
%% %
%% as $t \to \infty$ (see, for instance, in Section~13.75 of \cite{Watson}).   
%% Using the first term of this expression into (\ref{}) we obtain
%% the crude approximation
%% %
%% \begin{equation}
%% \end{equation}
%% %


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{Riccati's equation, Kummer's equation and phase functions}

In this section, we suppose that $q$ is a smooth, real-valued function defined on an open
interval $I \subset \mathbb{R}$.
In the event that $q$ is strictly negative on $I$, 
two linearly independent solutions of  the second order differential equation
\begin{equation}
y''(t) + q(t) y(t) = 0 \ \ \mbox{for all}\ \ t \in I
\label{preliminaries:riccati:diffeq}
\end{equation}
%
both of which are positive on $I$ can be found.   This follows easily
from standard proofs of Picard's theorem 
on the existence and uniqueness of solutions of ordinary differential
equations  (see, for instance, Section~2.3 of \cite{Hille}).
Any positive solution $y$ of (\ref{preliminaries:riccati:diffeq})
can be represented in the form $y=\exp(r(t))$ with $r$ real-valued, and a straightforward
computation shows that $r$ must satisfy
%
\begin{equation}
r''(t)  + (r'(t))^2 + q(t) = 0
\ \ \mbox{for all}\ \ t \in I.
\label{preliminaries:riccatieq}
\end{equation}
%
Equation~(\ref{preliminaries:riccatieq}) is known as Riccati's equation;
a detailed discussion of it can be found in \cite{Hille}, among
many other sources.  


When $q$ is positive on $I$, 
the solutions of  (\ref{preliminaries:riccati:diffeq}) oscillate and their logarithms
are complex-valued.   
In this case it is convenient to represent
them via a phase function.
We say that a smooth function $\alpha$ defined on $I$
is a phase function  for the second order differential equation
(\ref{preliminaries:riccati:diffeq})
provided $\alpha'$ does not vanish on $I$ and the pair
%
\begin{equation}
u(t) = \frac{\cos\left(\alpha(t)\right)}{\sqrt{\left|\alpha'(t)\right|}}
\label{preliminaries:riccati:u}
\end{equation}
%
and
%
\begin{equation}
v(t) = \frac{\sin\left(\alpha(t)\right)}{\sqrt{\left|\alpha'(t)\right|}}
\label{preliminaries:riccati:v}
\end{equation}
%
form a basis in the space of solutions of (\ref{preliminaries:riccati:diffeq}).    
Of course, from (\ref{preliminaries:riccati:u}) and (\ref{preliminaries:riccati:v}),
it is immediate that $\alpha$ is   simply the imaginary part of the logarithm
of the solution $u(t) + i v(t)$.   We do not use a phase function
to represent solutions of (\ref{preliminaries:riccati:diffeq})
in intervals on which $q$ is negative since in that event
the phase function cannot be efficiently represented
via polynomial expansions (see Figure~\ref{figure1}).
 
Proofs of the following elementary
results  regarding phase functions can be found in
\cite{Heitman-Bremer-Rokhlin-Vioreanu} and \cite{BremerBessel}.

\vskip 1em
\begin{theorem}
Suppose that $I$ is an open interval in $\mathbb{R}$, and that
$q$ is a smooth, real-valued function defined on $I$.  Suppose also
that $\alpha$ is a smooth, real-valued function defined on $I$ whose
first derivative does not vanish there.  Then $\alpha$
is a phase function for the second order differential
equation (\ref{preliminaries:riccati:diffeq}) if and only if
its derivative $\alpha'$
 satisfies the second order nonlinear differential equation
%
\begin{equation}
 q(t) 
- (\alpha'(t))^2
- \frac{1}{2}\left(\frac{\alpha'''(t)}{\alpha'(t)}\right)
+ \frac{3}{4}
\left(\frac{\alpha''(t)}{\alpha'(t)}\right)^2 = 0
\ \ \mbox{for all}\  \ t\in I.
\label{preliminaries:riccati:kummer}
\end{equation}
%
\label{theorem1}
\end{theorem}


\vskip 1em
\begin{theorem}
Suppose that $u,v$ is a pair of smooth, real-valued solutions
of (\ref{preliminaries:riccati:diffeq}) whose (necessarily constant)
Wronskian $W$ is nonzero.  Then  there is a phase function $\alpha$
for (\ref{preliminaries:riccati:diffeq}) such that
%
\begin{equation}
u(t) = \sqrt{W} \frac{\cos(\alpha(t)) }{\sqrt{|\alpha'(t)|}}
\label{preliminaries:riccati:u2}
\end{equation}
%
and
%
\begin{equation}
v(t) =  \sqrt{W}  \frac{\sin(\alpha(t)) }{\sqrt{|\alpha'(t)|}}.
\label{preliminaries:riccati:v2}
\end{equation}
%
Moreover, the derivative of $\alpha$ is given by
%
\begin{equation}
\alpha'(t) = \frac{W}{(u(t))^2 + (v(t))^2}
\ \ \mbox{for all} \ \ t \in I,
\end{equation}
%
and $\alpha$ is unique up to addition by an integer
multiple of $2\pi$.   That is, $\tilde{\alpha}$ is a phase
function for (\ref{preliminaries:riccati:diffeq}) 
such that (\ref{preliminaries:riccati:u2}) and (\ref{preliminaries:riccati:v2})
hold  if and only there exists an integer $L$ such that
%
\begin{equation}
\tilde{\alpha}(t) = \alpha(t) + 2\pi L
\ \ \mbox{for all} \ \ t \in I.
\end{equation}
%
\label{theorem2}
\end{theorem}


We will refer to (\ref{preliminaries:riccati:kummer}) as Kummer's equation,
after E.~E.~Kummer who studied it in \cite{Kummer}.  

\label{preliminaries:riccati}
\end{subsection}


%% %% Formula~(\ref{introduction:p}) is highly conducive to the numerical
%% %% calculation of Gauss-Jacobi quadrature rules.  

%% %% %% {\bf must do points, not coefficients}
%% %% %% bivariate piecewise Chebyshev expansions.  Because they are smooth,
%% %% a relatively small number of coefficients give high accuracy.
%% %% For example, when $N_{\mbox{\tiny max}} = 2^{16}$, 
%% %% The cost of computing the phase and amplitude functions is surpringly
%% %% low; indeed, for most values of $N_{\mbox{\tiny max}}$ it is faster
%% %% than the 
%% %% Once the phase and amplitude have been constructed, the 


%% %% where $P_\nu^{(a,b)}$ is a solution of Jacobi's differential equation
%% %% Since these functions are,
%% %% this procedure is surprisingly inexpensive.  Indeed,

%% %% Jacobi polynomials $P_\nu^{(a,b)}$ for $t \in (0,\pi)$ and $\dnu$
%% %% in the interval $(1,N_{\mbox{\tiny max}})$ with 
%% %% specified by the user.
%% %
%% %

%% %% For the most part, we do not have rigorous bounds on the asymptotic complexity of our
%% %% methods.    The running times of the algorithms described in this article
%% %% depend on the ranks of 
%% %% certain  matrices discretizing the nonscillatory phase function for Jacobi's differential
%% %% equation.  The estimation of these ranks appears to be difficult and 
%% %% However, several well-known algorithms such as the spherical harmonic transform
%% %% of \cite{TygertIII} depend on similar properties and 
%% %% {\bf here}

%% %% Our main basis of comparison are the algorithms of \cite{} for the calculation
%% %% of Gauss-Jacobi quadrature rules and the numerical evaluation,
%% %% and of \cite{Slevinsky1} for the application of the Chebyshev-Jacobi transform
%% %% and its inverse.  The Jacobi-Chebyshev transform is the mapping which
%% %% takes

%% %% {\bf not much literature on the numerical evaluation of 
%% %% Jacobi polynomials ... as distinct from the construction of asymptotic
%% %% expansions which may or may not lead to fast numerical algorithms.  mention difficulties
%% %% with expansions}



%% %% The numerical evaluation of Jacobi polynomials in time independent of degree
%% %% {\bf recurrence relations not useful; not many existing approaches;
%% %% Liouville-Green expansions not useful}

%% The remainder of this article is structured as follows.
%% In Section~\ref{section:preliminaries}, we 


%% the 
%% %
%% \begin{equation}
%% \psi(x,t),
%% \end{equation}
%% %
%% where $\psi$ is the nonoscillatory phase representing the solutions
%% of Jacobi's differential equation.  In particular, $\psi$ is related
%% to the Jacobi polynomial $P_\nu^{(a,b)}$ through the formula
%% %
%% \begin{equation}
%% P_\nu^{(a,b)}(x) = \frac{\cos()}{}
%% \end{equation}
%

%% It has been conjectured that these ranks grow logarithmically with
%% In this case, the running time of 
%% As the numerical experiments of this paper demonstratre, the 
%% {\bf cite MArk's conjecture}
%% Our algorithm 

%% Few algorithms for the numerical evaluation of Jacobi polynomials which
%% run in time independent of degree  
%% {\bf not true --- Townsend-Ale incude one; also mention Legendre approach
%% of the othre guys}


%% %% Speed not optimal
%% %% We user a variant of 
%% %% the algorithm of \cite{BremerKummer} for the numerical
%% %% This procedure is startingly efficient; indeed,
%% %% the total precomputation time is comparable to the cost
%% %% to apply the \cite{Slevinsky}


%% The Jacobi polynomials form an orthonormal basis
%% in the weighted Lebesgue space 
%% %
%% $$L^2\left((-1,1); (1-x)^a (1+x)^b\right)$$
%% %
%% {\bf change of variables}
%% %
%% %% In this article, we focus on the case in which $a$ and $b$
%% %% in the interval $(-1/2,1/2)$.  In fact, our algorothms work in slightly more
%% %% generality and can when $a$, $b$ > $1/2$, although they will fail for
%% %% sufficiently large values of $a$ and $b$.

%% The most well-developed algorithms for forming and manipulating
%% Jacobi expansions are dure 
%% {\bf well there is probably Roklin butterfly}
%% {\bf butterfly transforms for Jacobi??}
%% %

%% \begin{equation}
%% f(x) = \sum_{
%% \end{equation}
%

%% existing algorithms for forming and  in terms of Jacobi polynomials in general
%% leaves much 

%%   Generally speaking, there are
%% three components needed to make such an approach viale.
%% zeros/quadrature rules, evaluation of functions, fast transform

%% Discrete Sturm-Liouville eigentransforms are widely used in numerical analysis.


%% Discrete Sturm-Liouville eigentransforms are ubi


%% Second order differential equations with nonoscillatory coefficients admit
%% nonoscillatory phase functions \cite{DLMF,Bremer-Rokhlin,Heitman-Bremer-Rokhlin}.


%% It is well known that many familimi

%% %% The Jacobi polynomials 

%% %% It is well-known that many second order differential equations admit
%% %% nonoscillatory phase functions.  Bessel's equation is one well-known

%% %% Here, we describe a 
 
%% %% Jacobi's differential equation is 
%% %% %
%% %% \begin{equation}
%% %% (1-x^2) \psi''(x)  + (b-a - (a+b+2)x)\psi'(x) + \nu(\nu+a+b+1)\psi(x) = 0.
%% %% \label{introduction:jacobi}
%% %% \end{equation}
%% %% %
%% %% When $-\frac{1}{2} < a, b < \frac{1}{2}$, which is the regime we will consider
%% %% here, the solutions of (\ref{introduction:jacobi})
%% %% are oscillatory on the interval $(-1,1)$.  If, in addition, the parameter $\nu$ is large,
%% %% the solutions of Jacobi's equation are highly oscillatory.  This makes
%% %% most brute force algorithms for the evaluation of the solutions of (),
%% %% their and their .

% %% {\bf asymptotic estimates algorithms of  Hale and Townsend}

%% %% It is well known that the solutions of the first kind, which we will denote by
%% %% $P_\nu^{a,b}$, form an orthonormal basis in the weighted Lebesgues space
%% %% $L^2$.

%% %% It is well known that many second order differential equations, such
%% %% Bessel's differential equation and Jacobi's differential equation,
%% %% admit nonoscillatory phase functions.  That is, under a simple
%% %% change of variables, each of their solutions can be represented in the
%% %% form
%% %% %
%% %% \begin{equation}
%% %% a_1 \frac{\cos(\alpha(t))}{\sqrt{\alpha'(t)}} + 
%% %% a_2 \frac{\sin(\alpha(t))}{\sqrt{\alpha'(t)}}
%% %% \end{equation}
%% %% %
%% %% where $\alpha$ is a nonoscillatory function.  In \cite{Bremer-Rokhlin}
%% %% and \cite{Heitman-Bremer-Rokhlin}, it is shown that this property
%% %% is, in fact,  possesed by a large class of differential
%% %% equations whose coefficients are nonoscillatory.  

%% %% Among
%% %% other things, this implies that many Sturm-Liouville eigenfunction
%% %% transforms are
%% %% %
%% %% \begin{equation}
%% %% \int_a^b \varphi(t,\lambda) \exp(i \psi(t,\lambda)\ f(t) dt
%% %% \end{equation}
%% %

%% %% %

%% %% \begin{equation}
%% %% \left\{
%% %% \begin{aligned}
%% %% p(t) y''(t) + p'(t) y'(t) + \left( q(t)  \lambda w(t)\right) y(t) = 0 \ \ \mbox{for all} \ \ a <t < b \\
%% %% \cos(\gamma_1) y(a) + \sin(\gamma_2) y'(a) = 0 \\
%% %% \gamma_1 y(a) + \gamma_2 y'(a) = 0 \\
%% %% \end{aligned}
%% %% \right.
%% %% \end{equation}
%% %

%% Overview of Sturm-Liouville eigenfunctions

%% Nonoscillatory Phase functions

%% Butterfly algorithms

%% outline of paper


%% Butterfly algorithms are a collection of techniques for the numerical
%% application of certain classes of oscillatory integral operators.
%% Including Fourier integral operators

%% Unfortuantely, in some cases that  code loses a small amount of accuracy when 
%% evaluating  quadrature weights  corresponding to quadrature nodes near the points $\pm 1$.
%% Interestingly,
%% the MATLAB implementation of the Hale-Townsend algorithm 
%% included with the Chebfun package \cite{chebfun} 
%% does not suffer from this defect.  Accordingly, we omitted the $20$ quadrature nodes closest
%% to each of the points $\pm 1$ when measuring the accuracy of the weights
%% returned by our algorithm through comparison with the those generated by
%% \cite{Hale-Townsend-Code}.


==> tablebrute.tex <==
 \begin{tabular}{lccc}
 \toprule
 $n$   & Forward Jacobi   & Brute force             & Ratio  \\
       & transform time    & transform time &  \\
       & algorithm of Section~\ref{section:transform} & &   \\
 \midrule
100 & 1.16\e{-02} & 3.91\e{-04} & 3.36\e{-02}  \\
100 & 7.28\e{-03} & 3.29\e{-04} & 4.52\e{-02}  \\
128 & 7.98\e{-03} & 6.00\e{-04} & 7.51\e{-02}  \\
256 & 1.28\e{-02} & 2.95\e{-03} & 2.29\e{-01}  \\
512 & 1.63\e{-02} & 1.42\e{-02} & 8.69\e{-01}  \\
1\sep,024 & 2.39\e{-02} & 7.70\e{-02} & 3.20\e{+00}   \\
2\sep,048 & 2.67\e{-02} & 2.86\e{-01} & 1.06\e{+01}   \\
4\sep,096 & 4.23\e{-02} & 1.22\e{+00}  & 2.89\e{+01}   \\
 \bottomrule
 \end{tabular}

